A Design-Space Exploration for Allocating Security Tasks in Multicore Real-Time Systems

The increased capabilities of modern real-time systems (RTS) expose them to various security threats. Recently, frameworks that integrate security tasks without perturbing the real-time tasks have been proposed, but they only target single core systems. However, modern RTS are migrating towards multicore platforms. This makes the problem of integrating security mechanisms more complex, as designers now have multiple choices for where to allocate the security tasks. In this paper we propose HYDRA, a design space exploration algorithm that finds an allocation of security tasks for multicore RTS using the concept of opportunistic execution. HYDRA allows security tasks to operate with existing real-time tasks without perturbing system parameters or normal execution patterns, while still meeting the desired monitoring frequency for intrusion detection. Our evaluation uses a representative real-time control system (along with synthetic task sets for a broader exploration) to illustrate the efficacy of HYDRA.

==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

# LATEX = pdflatex 
LATEX = xelatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> Sections/app_esearch.tex <==

\subsection{Comparison with Optimal Solution} \label{appendix:esearch}

\begin{figure}[!t]
\centering
\includegraphics[scale=0.40]{esearch_2.pdf}
\caption{Comparing \coolnameplus with optimal solution: we consider $M=2$ and $N_S \in [2, 6]$ with other parameters similar to that mentioned in Section \ref{subsubsec:setup}.} 
\label{fig:esearch}
\end{figure}

In Fig. \ref{fig:esearch} we empirically compared \coolnameplus with an optimal solution where we exhaustively searched for all possible combinations for a small setup\footnote{Recall that there are $|\mathcal{M} \times \Gamma_s|$ different combinations possible. As an example, for a moderately small system with $M=4, N_S = 10$, there are $1048576
$ different combinations to choose from where for each combination the periods could be any value within the range $[T_s^{des}, T_s^{max}]$.}. The x-axis of Fig. \ref{fig:esearch} represents total system utilization and y-axis is the difference in cumulative tightness (\eg $\Delta_{\eta} = \frac{\eta_{\rm OPT} - \eta_{\rm HYDRA}}{\eta_{\rm OPT}}\times 100 \%$) %$\sum\limits_{\tau_s \in \Gamma_S} \eta_s$) 
for \coolnameplus and optimal solution. As shown in the figure for low to medium utilization cases \coolnameplus performs similar to that of the optimal solution (\eg the difference is zero). However for higher utilizations performance degrades. This is because \coolnameplus follows a iterative best-fit strategy to find the periods (and assignment). Hence for higher utilization values the lower priority tasks may not get period close to the desired one (and the cumulative tightness degrades). As we see from the figure, the degradation (in cumulative tightness) is no more than $22\%$ and that may be acceptable given the computational impracticality of finding an optimal solution.

